Density Functional Leveraged Tight-binding Insights into Inorganic Halide Perovskites

Compared to first principles studies like DFT (physically accurate, computationally expensive), the TB approach allows the disentanglement of the region of interest, to wit the fermi level. This allows the creation of simplified, highly interpretable models that give chemically grounded insights. In this paper we employ a Wannierized TB approach to tune the bandgap and electronic structure via anion exchange and investigate its impact on the orbital interactives of inorganic lead halide perovskites. Further adjustment of the hopping norm and maximum distance leads to a reduced TB model which regenerates the broad features of the band structure with a fraction of the parameters, thereby making the model simpler and highly interpretable. We observe that due to the asymmetry of the unit cell and the delocalized nature of its orbitals, CsPbBrI2 follows a many-small hopping scheme different in character from the few-big strategy taken by the other perovskites. Finally we leverage the TB model to study the electronic and thermal transport properties of these materials. These insight enable the identification of optimal doping strategies that could enhance thermoelectric performance by improving carrier mobility or optimizing the Seebeck coefficient.

==> DAG.tex <==
% \begin{center}
%     \begin{tikzpicture}[
%     grow=right,
%     level distance=200mm,
%     sibling distance=105mm]
        
%         \node (A) at (0, 0){Electronegativity};
%         \node (B) at (4, 0) {Cell symmetry};
%         \node (C) at (0,-2) {Cell Volume};
%         \node [text width=2.1cm, align=center] (D) at (4,-2) {Orbital localization};
%         \node (F) at (5,-3.5) {\bf{Bandgap}} ;
    
%         \path [->](A) edge node[right] {} (B);
%         \path [->](A) edge node[right] {} (C);
%         \path [->](B) edge node[right] {} (D);
%         \path [->](B) edge node[right] {} (C);
%         \path [->](C) edge node[right] {} (D); 
%         \path [->](D) edge node[right] {} (F); 
%     \end{tikzpicture}
% \end{center}


==> _figs/article/w90orbs.tex <==



\begin{figure}[ht!] % Figure placement
    \centering
    \begin{subfigure}[t]{0.22\textwidth} % Subfigure 1
        \centering
        \includegraphics[width=\textwidth]{_figs/article/Pb_xsf.png}
        \caption{}
        \label{Pborb}
    \end{subfigure}
    \hspace{0.5cm} % Horizontal spacing
    \begin{subfigure}[t]{0.22\textwidth} % Subfigure 2
        \centering
        \includegraphics[width=\textwidth]{_figs/article/px_xsf.png}
        \caption{}
        \label{p1}
    \end{subfigure}
    \hspace{0.5cm} % Horizontal spacing
    \begin{subfigure}[t]{0.22\textwidth} % Subfigure 3
        \centering
        \includegraphics[width=\textwidth]{_figs/article/py_xsf.png}
        \caption{}
        \label{p2}
    \end{subfigure}
    \hspace{0.5cm} % Horizontal spacing
    \begin{subfigure}[t]{0.22\textwidth} % Subfigure 4
        \centering
        \includegraphics[width=\textwidth]{_figs/article/pz_xsf.png}
        \caption{}
        \label{p3}
    \end{subfigure}
    
    \caption{ Wannier orbitals (light blue and yellow isosurfaces)  on a \(3\times3\times3\) supercell of \Briii\ (Cs: pink, Pb: dark gray, Br: light purple) are shown for (a) Pb-p orbital (b-d) Br p-orbitals. }
    \label{w90orbs}
\end{figure}
